Mass assembly and morphological transformations since $z\sim3$ from CANDELS

[abridged] We quantify the evolution of the stellar mass functions of star-forming and quiescent galaxies as a function of morphology from $z\sim 3$ to the present. Our sample consists of ~50,000 galaxies in the CANDELS fields ($\sim880$ $arcmin^2$), which we divide into four main morphological types, i.e. pure bulge dominated systems, pure spiral disk dominated, intermediate 2-component bulge+disk systems and irregular disturbed galaxies. Our main results are: Star-formation: At $z\sim 2$, 80\% of the stellar mass density of star-forming galaxies is in irregular systems. However, by $z\sim 0.5$, irregular objects only dominate at stellar masses below $10^9M\odot$. A majority of the star-forming irregulars present at $z\sim 2$ undergo a gradual transformation from disturbed to normal spiral disk morphologies by $z\sim 1$ without significant interruption to their star-formation. Rejuvenation after a quenching event does not seem to be common except perhaps for the most massive objects. Quenching: We confirm that galaxies reaching a stellar mass of $M_*\sim10^{10.8}M_\odot$ ($M^*$) tend to quench. Also, quenching implies the presence of a bulge: the abundance of massive red disks is negligible at all redshifts over 2~dex in stellar mass. However the dominant quenching mechanism evolves. At $z>2$, the SMF of quiescent galaxies above $M^*$ is dominated by compact spheroids. Quenching at this early epoch destroys the disk and produces a compact remnant unless the star-forming progenitors at even higher redshifts are significantly more dense. At $1<z<2$, the majority of newly quenched galaxies are disks with a significant central bulge. This suggests that mass-quenching at this epoch starts from the inner parts and preserves the disk. At $z<1$, the high mass end of the passive SMF is globally in place and the evolution mostly happens at stellar masses below $10^{10}M_\odot$.

==> tbl_fit_params_SF_Q.tex <==
& 0.2-0.5& 4465&  8.43& $10.68^{+0.09}_{-0.09}$ & $0.92^{+0.22}_{-0.22}$ & $-1.46^{+0.04}_{-0.04}$ &$ 7.85^{+0.05}_{-0.05}$& &0768&  8.60& $11.01^{+0.14}_{-0.14}$ & $0.56^{+0.14}_{-0.14}$ & $-1.09^{+0.06}_{-0.06}$ &$ 7.78^{+0.07}_{-0.07}$\\ 
& 0.5-0.8& 7032&  8.94& $10.92^{+0.07}_{-0.07}$ & $0.83^{+0.17}_{-0.17}$ & $-1.46^{+0.04}_{-0.04}$ &$ 8.05^{+0.04}_{-0.04}$& &1244&  9.04& $10.90^{+0.04}_{-0.04}$ & $1.47^{+0.16}_{-0.16}$ & $-0.68^{+0.05}_{-0.05}$ &$ 8.02^{+0.06}_{-0.06}$\\ 
& 0.8-1.1& 6743&  9.29& $10.93^{+0.06}_{-0.06}$ & $0.81^{+0.17}_{-0.17}$ & $-1.41^{+0.05}_{-0.05}$ &$ 8.01^{+0.03}_{-0.03}$& &0859&  9.48& $10.84^{+0.04}_{-0.04}$ & $1.17^{+0.11}_{-0.11}$ & $-0.40^{+0.08}_{-0.08}$ &$ 7.85^{+0.06}_{-0.06}$\\ 
& 1.1-1.5& 6534&  9.61& $10.98^{+0.06}_{-0.06}$ & $0.51^{+0.10}_{-0.10}$ & $-1.41^{+0.06}_{-0.06}$ &$ 7.86^{+0.03}_{-0.03}$& &0565&  9.79& $10.73^{+0.02}_{-0.02}$ & $0.64^{+0.04}_{-0.04}$ & $ 0.00^{+0.00}_{-0.00}$ &$ 7.53^{+0.05}_{-0.05}$\\ 
& 1.5-2& 6261& 10.02& $10.82^{+0.05}_{-0.05}$ & $0.93^{+0.15}_{-0.15}$ & $-1.00^{+0.12}_{-0.12}$ &$ 7.78^{+0.04}_{-0.04}$& &0541& 10.16& $10.78^{+0.03}_{-0.03}$ & $0.44^{+0.03}_{-0.03}$ & $ 0.00^{+0.00}_{-0.00}$ &$ 7.42^{+0.06}_{-0.06}$\\ 
& 2-2.5& 3961& 10.21& $11.29^{+0.16}_{-0.16}$ & $0.13^{+0.08}_{-0.08}$ & $-1.61^{+0.19}_{-0.19}$ &$ 7.72^{+0.03}_{-0.03}$& &0211& 10.51& $10.85^{+0.27}_{-0.27}$ & $0.18^{+0.08}_{-0.08}$ & $-0.56^{+0.86}_{-0.86}$ &$ 7.05^{+0.08}_{-0.08}$\\ 
& 2.5-3& 2057& 10.36& $11.02^{+0.17}_{-0.17}$ & $0.19^{+0.11}_{-0.11}$ & $-1.08^{+0.46}_{-0.46}$ &$ 7.33^{+0.05}_{-0.05}$& &0090& 11.05& $11.01^{+0.14}_{-0.14}$ & $0.56^{+0.14}_{-0.14}$ & $-1.09^{+0.06}_{-0.06}$ &$99.00^{+0.00}_{-0.00}$\\ 
& 0.2-0.5& 0418&  8.43& $15.58^{+****}_{-****}$ & $0.00^{+0.24}_{-0.24}$ & $-1.71^{+0.10}_{-0.10}$ &$ 7.00^{+0.09}_{-0.09}$& &0202&  8.60& $11.04^{+0.22}_{-0.22}$ & $0.28^{+0.09}_{-0.09}$ & $-0.96^{+0.08}_{-0.08}$ &$ 7.48^{+0.10}_{-0.10}$\\ 
& 0.5-0.8& 0798&  8.94& $14.37^{+****}_{-****}$ & $0.00^{+0.02}_{-0.02}$ & $-1.77^{+0.08}_{-0.08}$ &$ 7.18^{+0.05}_{-0.05}$& &0586&  9.04& $10.88^{+0.05}_{-0.05}$ & $0.85^{+0.10}_{-0.10}$ & $-0.61^{+0.06}_{-0.06}$ &$ 7.76^{+0.07}_{-0.07}$\\ 
& 0.8-1.1& 0872&  9.29& $10.86^{+0.14}_{-0.14}$ & $0.10^{+0.04}_{-0.04}$ & $-1.46^{+0.10}_{-0.10}$ &$ 7.05^{+0.07}_{-0.07}$& &0470&  9.48& $10.81^{+0.06}_{-0.06}$ & $0.62^{+0.07}_{-0.07}$ & $-0.41^{+0.10}_{-0.10}$ &$ 7.56^{+0.09}_{-0.09}$\\ 
& 1.1-1.5& 0928&  9.61& $10.72^{+0.11}_{-0.11}$ & $0.16^{+0.05}_{-0.05}$ & $-1.20^{+0.13}_{-0.13}$ &$ 6.98^{+0.06}_{-0.06}$& &0331&  9.79& $10.52^{+0.08}_{-0.08}$ & $0.39^{+0.03}_{-0.03}$ & $ 0.29^{+0.22}_{-0.22}$ &$ 7.18^{+0.08}_{-0.08}$\\ 
& 1.5-2& 0889& 10.02& $10.58^{+0.10}_{-0.10}$ & $0.27^{+0.05}_{-0.05}$ & $-0.38^{+0.30}_{-0.30}$ &$ 6.97^{+0.06}_{-0.06}$& &0316& 10.16& $10.35^{+0.07}_{-0.07}$ & $0.14^{+0.06}_{-0.06}$ & $ 1.68^{+0.48}_{-0.48}$ &$ 7.11^{+0.07}_{-0.07}$\\ 
& 2-2.5& 0568& 10.21& $11.00^{+0.29}_{-0.29}$ & $0.06^{+0.05}_{-0.05}$ & $-1.08^{+0.46}_{-0.46}$ &$ 6.83^{+0.09}_{-0.09}$& &0120& 10.51& $10.72^{+0.23}_{-0.23}$ & $0.13^{+0.02}_{-0.02}$ & $-0.14^{+1.02}_{-1.02}$ &$ 6.81^{+0.10}_{-0.10}$\\ 
& 2.5-3& 0248& 10.36& $15.58^{+****}_{-****}$ & $0.00^{+0.24}_{-0.24}$ & $-1.71^{+0.10}_{-0.10}$ &$ 6.20^{+0.15}_{-0.15}$& &0039& 11.05& $11.04^{+0.22}_{-0.22}$ & $0.28^{+0.09}_{-0.09}$ & $-0.96^{+0.08}_{-0.08}$ &$99.00^{+0.00}_{-0.00}$\\ 
& 0.2-0.5& 0233&  8.43& $10.53^{+0.12}_{-0.12}$ & $0.48^{+0.11}_{-0.11}$ & $-0.85^{+0.09}_{-0.09}$ &$ 7.18^{+0.11}_{-0.11}$& &0161&  8.60& $10.42^{+0.07}_{-0.07}$ & $0.94^{+0.13}_{-0.13}$ & $-0.17^{+0.13}_{-0.13}$ &$ 7.36^{+0.09}_{-0.09}$\\ 
& 0.5-0.8& 0408&  8.94& $10.66^{+0.06}_{-0.06}$ & $0.46^{+0.08}_{-0.08}$ & $-0.78^{+0.08}_{-0.08}$ &$ 7.28^{+0.09}_{-0.09}$& &0319&  9.04& $10.63^{+0.05}_{-0.05}$ & $0.89^{+0.08}_{-0.08}$ & $-0.01^{+0.11}_{-0.11}$ &$ 7.58^{+0.08}_{-0.08}$\\ 
& 0.8-1.1& 0360&  9.29& $10.94^{+0.10}_{-0.10}$ & $0.24^{+0.05}_{-0.05}$ & $-0.82^{+0.10}_{-0.10}$ &$ 7.28^{+0.09}_{-0.09}$& &0208&  9.48& $10.67^{+0.06}_{-0.06}$ & $0.43^{+0.04}_{-0.04}$ & $ 0.29^{+0.18}_{-0.18}$ &$ 7.37^{+0.09}_{-0.09}$\\ 
& 1.1-1.5& 0281&  9.61& $11.02^{+0.12}_{-0.12}$ & $0.11^{+0.03}_{-0.03}$ & $-0.82^{+0.13}_{-0.13}$ &$ 7.02^{+0.09}_{-0.09}$& &0113&  9.79& $10.57^{+0.08}_{-0.08}$ & $0.10^{+0.02}_{-0.02}$ & $ 1.29^{+0.36}_{-0.36}$ &$ 7.00^{+0.11}_{-0.11}$\\ 
& 1.5-2& 0196& 10.02& $10.91^{+0.16}_{-0.16}$ & $0.08^{+0.02}_{-0.02}$ & $-0.38^{+0.34}_{-0.34}$ &$ 6.78^{+0.12}_{-0.12}$& &0074& 10.16& $10.65^{+0.09}_{-0.09}$ & $0.03^{+0.02}_{-0.02}$ & $ 1.64^{+0.62}_{-0.62}$ &$ 6.77^{+0.12}_{-0.12}$\\ 
& 2-2.5& 0081& 10.21& $11.21^{+0.48}_{-0.48}$ & $0.01^{+0.01}_{-0.01}$ & $-1.06^{+0.69}_{-0.69}$ &$ 6.28^{+0.14}_{-0.14}$& &0010& 10.51& $10.56^{+0.72}_{-0.72}$ & $0.00^{+0.02}_{-0.02}$ & $ 1.94^{+4.85}_{-4.85}$ &$ 5.87^{+0.00}_{-0.00}$\\ 
& 2.5-3& 0028& 10.36& $10.53^{+0.12}_{-0.12}$ & $0.48^{+0.11}_{-0.11}$ & $-0.85^{+0.09}_{-0.09}$ &$ 6.66^{+0.06}_{-0.06}$& &0007& 11.05& $10.42^{+0.07}_{-0.07}$ & $0.94^{+0.13}_{-0.13}$ & $-0.17^{+0.13}_{-0.13}$ &$99.00^{+0.00}_{-0.00}$\\ 
& 0.2-0.5& 1263&  8.43& $10.33^{+0.07}_{-0.07}$ & $1.21^{+0.23}_{-0.23}$ & $-1.17^{+0.05}_{-0.05}$ &$ 7.46^{+0.06}_{-0.06}$& &0202&  8.60& $16.02^{+****}_{-****}$ & $0.00^{+3.45}_{-3.45}$ & $-1.55^{+0.11}_{-0.11}$ &$ 7.18^{+0.08}_{-0.08}$\\ 
& 0.5-0.8& 2162&  8.94& $10.66^{+0.08}_{-0.08}$ & $0.80^{+0.18}_{-0.18}$ & $-1.24^{+0.06}_{-0.06}$ &$ 7.65^{+0.05}_{-0.05}$& &0179&  9.04& $15.81^{+****}_{-****}$ & $0.00^{+1.22}_{-1.22}$ & $-1.54^{+0.14}_{-0.14}$ &$ 7.06^{+0.09}_{-0.09}$\\ 
& 0.8-1.1& 1752&  9.29& $10.80^{+0.07}_{-0.07}$ & $0.54^{+0.11}_{-0.11}$ & $-1.18^{+0.07}_{-0.07}$ &$ 7.59^{+0.04}_{-0.04}$& &0084&  9.48& $11.52^{+0.58}_{-0.58}$ & $0.02^{+0.02}_{-0.02}$ & $-1.17^{+0.22}_{-0.22}$ &$ 6.85^{+0.11}_{-0.11}$\\ 
& 1.1-1.5& 1126&  9.61& $11.01^{+0.10}_{-0.10}$ & $0.14^{+0.04}_{-0.04}$ & $-1.30^{+0.09}_{-0.09}$ &$ 7.27^{+0.06}_{-0.06}$& &0044&  9.79& $11.15^{+0.26}_{-0.26}$ & $0.02^{+0.01}_{-0.01}$ & $-0.60^{+0.38}_{-0.38}$ &$ 6.48^{+0.16}_{-0.16}$\\ 
& 1.5-2& 0748& 10.02& $10.84^{+0.12}_{-0.12}$ & $0.13^{+0.04}_{-0.04}$ & $-0.96^{+0.21}_{-0.21}$ &$ 6.96^{+0.08}_{-0.08}$& &0039& 10.16& $10.79^{+0.43}_{-0.43}$ & $0.04^{+0.01}_{-0.01}$ & $-0.11^{+1.01}_{-1.01}$ &$ 6.36^{+0.13}_{-0.13}$\\ 
& 2-2.5& 0299& 10.21& $15.81^{+****}_{-****}$ & $0.00^{+0.05}_{-0.05}$ & $-1.76^{+0.43}_{-0.43}$ &$ 6.77^{+0.09}_{-0.09}$& &0014& 10.51& $11.25^{+0.46}_{-0.46}$ & $0.01^{+0.00}_{-0.00}$ & $ 0.07^{+1.28}_{-1.28}$ &$ 6.24^{+0.02}_{-0.02}$\\ 
& 2.5-3& 0103& 10.36& $10.33^{+0.07}_{-0.07}$ & $1.21^{+0.23}_{-0.23}$ & $-1.17^{+0.05}_{-0.05}$ &$ 6.32^{+0.07}_{-0.07}$& &0002& 11.05& $16.02^{+****}_{-****}$ & $0.00^{+3.45}_{-3.45}$ & $-1.55^{+0.11}_{-0.11}$ &$99.00^{+0.00}_{-0.00}$\\ 
& 0.2-0.5& 2472&  8.43& $10.15^{+0.15}_{-0.15}$ & $0.40^{+0.19}_{-0.19}$ & $-1.71^{+0.09}_{-0.09}$ &$ 7.11^{+0.05}_{-0.05}$& &0192&  8.60& $14.48^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & $-2.07^{+0.19}_{-0.19}$ &$ 6.05^{+0.03}_{-0.03}$\\ 
& 0.5-0.8& 3460&  8.94& $10.56^{+0.11}_{-0.11}$ & $0.31^{+0.11}_{-0.11}$ & $-1.66^{+0.07}_{-0.07}$ &$ 7.40^{+0.04}_{-0.04}$& &0130&  9.04& $16.17^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & $-1.92^{+0.16}_{-0.16}$ &$ 6.21^{+0.18}_{-0.18}$\\ 
& 0.8-1.1& 3532&  9.29& $10.72^{+0.10}_{-0.10}$ & $0.33^{+0.11}_{-0.11}$ & $-1.57^{+0.08}_{-0.08}$ &$ 7.51^{+0.03}_{-0.03}$& &0081&  9.48& $18.87^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & $-1.57^{+0.21}_{-0.21}$ &$ 6.53^{+0.10}_{-0.10}$\\ 
& 1.1-1.5& 3887&  9.61& $10.86^{+0.09}_{-0.09}$ & $0.23^{+0.07}_{-0.07}$ & $-1.57^{+0.08}_{-0.08}$ &$ 7.50^{+0.04}_{-0.04}$& &0048&  9.79& $20.15^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & $-1.45^{+0.19}_{-0.19}$ &$ 6.47^{+0.11}_{-0.11}$\\ 
& 1.5-2& 4132& 10.02& $10.88^{+0.08}_{-0.08}$ & $0.37^{+0.10}_{-0.10}$ & $-1.28^{+0.14}_{-0.14}$ &$ 7.54^{+0.03}_{-0.03}$& &0065& 10.16& $19.21^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & $-1.59^{+0.19}_{-0.19}$ &$ 6.64^{+0.12}_{-0.12}$\\ 
& 2-2.5& 2776& 10.21& $10.93^{+0.06}_{-0.06}$ & $0.24^{+0.04}_{-0.04}$ & $-1.28^{+0.00}_{-0.00}$ &$ 7.41^{+0.05}_{-0.05}$& &0038& 10.51& $17.85^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & $-1.93^{+0.39}_{-0.39}$ &$ 6.61^{+0.04}_{-0.04}$\\ 
& 2.5-3& 1530& 10.36& $11.53^{+0.37}_{-0.37}$ & $0.03^{+0.04}_{-0.04}$ & $-1.67^{+0.35}_{-0.35}$ &$ 7.37^{+0.04}_{-0.04}$& &0023& 11.05& $14.48^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & $-2.07^{+0.19}_{-0.19}$ &$99.00^{+0.00}_{-0.00}$\\ 

